Reroute, Don't Remove: Recoverable Visual Token Routing for Vision-Language Models

Vision-language models (VLMs) project images into hundreds to thousands of visual tokens, making decoder inference expensive in both attention computation and KV-cache memory. Existing visual-token reduction methods largely follow a rank-and-remove paradigm: they score visual tokens, keep a compact subset, and permanently discard the rest. We show that this irreversible action is fragile because visual-token importance changes across decoder depth; tokens ranked low at one stage may become relevant in later layers, especially for grounding-sensitive queries. We propose Reroute, a training-free plug-in that replaces removal with recoverable routing. At each routing stage, selected vision tokens pass through decoder blocks, while deferred tokens bypass the stage and re-enter the candidate pool at the next routing decision. Reroute reuses existing attention-score ranking rules and stage-wise schedules, preserving the theoretical TFLOPs and KV-cache budget class of the pruning method it augments. Across FastV, PDrop, and N\"uwa variants on LLaVA-1.5 and Qwen backbones, reroute improves grounding under aggressive token reduction while maintaining general VQA performance. These results suggest that VLM token reduction should not be viewed only as irreversible pruning, but also as recoverable routing. The code can be found here: https://github.com/elmma/mllm-reroute/

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1--2 sentence) justification right after your answer (even for \answerNA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will also be asked to include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While \answerYes{} is generally preferable to \answerNo{}, it is perfectly acceptable to answer \answerNo{} provided a proper justification is given (e.g., error bars are not reported because it would be too computationally expensive'' or ``we were unable to find the license for the dataset we used''). In general, answering \answerNo{} or \answerNA{} is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We state that Reroute is a training-free recoverable visual-token routing method that replaces irreversible removal with deferral while preserving the matched theoretical budget of the pruning baseline. Our method formulation and experiments across LLaVA-1.5 and Qwen-family backbones support this scope under matched token budgets.

    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We include a limitations paragraph covering the dependence on the attention-score router, sensitivity to overly aggressive budgets, the gap between theoretical efficiency and practical latency, the lack of exhaustive combinations with other compression methods, and unresolved interactions with hybrid linear-attention architectures.
 architectures.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not present formal theoretical results requiring proofs. The equations in the paper define the algorithmic formulation and budget-matching setup rather than theorems or lemmas.

    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide the main reproducibility details needed to understand and reproduce the evaluation protocol, including lmms-eval usage, task identifiers, evaluation splits, metrics, model families, inference settings, prompt and post-processing conventions, and routing/pruning configurations. Reproduction assumes access to the same public models, datasets, and evaluation framework.

    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We evaluate on public benchmark datasets and public pretrained VLM checkpoints, and we provide the experimental protocol and routing configurations needed to reproduce the evaluation setup. However, we do not include an open code release as part of the anonymous submission; we plan to release the code upon acceptance.


    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our method is training-free, so optimizer and training hyperparameters are not applicable. We specify the datasets, splits, metrics, model checkpoints/backbones, lmms-eval settings, prompt and post-processing conventions, routing layers, keep-ratio calibration, and position-index handling used in the experiments.


    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We report deterministic benchmark scores and normalized ratios, but we do not provide error bars, confidence intervals, bootstrap estimates, or statistical significance tests. This is a limitation of the current experimental reporting.

    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Appendix A.2 states that all experiments are conducted on a single NVIDIA RTX 4090 GPU. Table 4 reports TFLOPs and KV-cache memory measurements normalized against the vanilla baseline.

    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: To the best of our knowledge, our research conforms with the NeurIPS Code of Ethics. We evaluate a training-free efficiency method on existing public VLM backbones and established benchmarks, without collecting private data, conducting human-subject studies, or releasing a high-risk generative model.

    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: To the best of our knowledge, our method does not provide direct paths for825negative applications

    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not introduce or release a new high-risk pretrained model, image generator, scraped dataset, or human-data asset. Our contribution is a training-free inference-time routing method evaluated on existing models and public benchmarks.


    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All used assets are publicly released and properly cited: LLaVA-1.5-7B [42], Qwen2.5-VL-7B [6], Qwen3.5-9B [54], the RefCOCO/RefCOCO+/RefCOCOg benchmarks [30, 79], and the VQA benchmarks (GQA [27], TextVQA [59], MME [18], MMBench [46], MMMU [80], POPE [36], ScienceQA [49], SEEDBench [33]). FastV [12], PDrop [71], and Nüwa [26] baselines are cited; we use the official Nüwa codebase as noted in Section 5.1.

    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not introduce a new dataset, pretrained model checkpoint, or benchmark asset.


    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not conduct crowdsourcing experiments or human-subject research. All experiments are conducted on existing benchmarks and pretrained VLMs.

    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not conduct human-subject research or collect new participant data. Therefore IRB approval or equivalent review is not applicable.

    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: LLMs were not used as an important, original, or non-standard component of the core method. The proposed Reroute mechanism operates on visual tokens within VLM decoders using attention-score-based routing, which is the standard inference-time computation of the underlying models. Any LLM use was limited to writing/editing assistance and did not impact the methodology or originality of the research.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> sections/01_introduction.tex <==
\vspace{-2mm}
\section{Introduction}
\vspace{-2mm}

Vision-language models (VLMs)~\cite{liu2023visual,bai2023qwen} convert images into hundreds to thousands of visual tokens and feed them into a language-model decoder, making inference expensive in both attention computation and KV-cache storage. Decoder-side visual-token reduction has therefore become an important direction for scalable VLM deployment~\cite{chen2024image,xing2024pyramiddrop,huang2026n}.

Most existing methods follow a \emph{rank-and-remove} paradigm. Vision-encoder-side methods compress tokens before the decoder~\cite{yang2025visionzip,shang2025llava}, while decoder-side methods such as FastV~\cite{chen2024image}, PDrop~\cite{xing2024pyramiddrop}, FEATHER~\cite{endo2025feather}, and Nüwa~\cite{huang2026n} rank visual tokens inside the LLM using attention- or structure-aware scores. Despite differences in scoring and scheduling, their post-scoring action is the same: low-ranked tokens are permanently removed and cannot contribute to later layers.

This irreversible design assumes that visual-token importance is stable across decoder depth. Our analysis shows otherwise. As shown in Figure~\ref{fig:motivation}, shallow layers often attend diffusely, while target-relevant visual evidence emerges only in middle or deep layers. For example, a ground-truth token corresponding to ``man in green shirt'' has low attention percentiles at early pruning layers, causing FastV and PDrop to remove it, but later rises to the top percentile at deeper layers. Under aggressive reduction, this early irreversibility leads to grounding collapse, with IoU dropping below 0.4 across multiple backbones (Figure~\ref{fig:teaser}).

We argue that the limitation lies not in the scorer itself, but in the irreversible \emph{remove} action after scoring. We propose \textbf{Reroute}, a training-free plug-in that replaces permanent pruning with recoverable stage-wise routing. At each routing layer, Reroute reuses the existing text-to-vision attention score to select a top-$r$ fraction of visual tokens for Attn+FFN computation. The remaining tokens are not deleted; instead, they bypass the current stage and re-enter the candidate pool at the next routing layer, where they are re-ranked together with the full visual-token set. Thus, a token deferred at an early layer can be re-admitted later if its relevance increases.

Reroute preserves the theoretical FLOPs and KV-cache budget of the pruning baseline it augments, since only selected tokens participate in decoder computation at each routed stage. Conceptually, it instantiates mixture-of-depth-style conditional computation~\cite{raposo2024mixture} for VLM visual tokens without training a router, unlike learned-router methods such as $\gamma$-MoD~\cite{luo2024gamma}. We validate Reroute as a drop-in augmentation of FastV, PDrop, and Nüwa across LLaVA-1.5-7B, Qwen2.5-VL-7B, and Qwen3.5-9B, with the largest gains in grounding-heavy and aggressive-reduction regimes.

Our contributions are:
\begin{itemize}
    \item \textbf{Recoverable routing for visual-token reduction.} We formulate decoder-side visual-token pruning as stage-wise routing with deferred-token bypass, making conventional pruning a special case where deferred tokens are never re-admitted.
    \item \textbf{Training-free plug-in with matched efficiency.} Reroute reuses existing attention-based scorers and pruning schedules, introduces no trainable parameters, and preserves the theoretical FLOPs and KV-cache budget of the baseline method.
    \item \textbf{Consistent improvements across methods and backbones.} When applied to FastV, PDrop, and Nüwa, Reroute improves quality at matched budgets on VQA and grounding benchmarks, with \textbf{Nüwa+Reroute achieving the strongest grounding-oriented performance} in our evaluation.
\end{itemize}

==> sections/02_related.tex <==
\section{Related Work}
\label{sec:intro}

placeholder

==> tables/llava_efficiency.tex <==
% ============================================================
% Required packages
% ============================================================
% \usepackage{booktabs}
% \usepackage[table]{xcolor}
% \usepackage{array}

% ============================================================
% Macros / colors
% ============================================================
\providecommand{\na}{--}
\newcommand{\effdown}[1]{\textcolor{green!55!black}{$\downarrow$ #1\%}}

\definecolor{vanillarow}{HTML}{EFEFEF}
\definecolor{baserow}{HTML}{FFF7E6}
\definecolor{routerow}{HTML}{EAF6EA}

% ============================================================
% Efficiency Table
% ============================================================
\begin{table}[t]
\centering
\caption{
\textbf{Efficiency comparison on LLaVA-1.5-7B under different average visual-token budgets.}
TFLOPs and KV-cache memory are reported for the main decoder computation and normalized against the vanilla full-token baseline.
}
\label{tab:efficiency_comparison}

\vspace{0.45em}

\footnotesize
\setlength{\tabcolsep}{6.2pt}
\renewcommand{\arraystretch}{0.96}
\setlength{\aboverulesep}{0.25ex}
\setlength{\belowrulesep}{0.25ex}
\setlength{\cmidrulesep}{0.12ex}

\begin{tabular}{@{}l c cc cc@{}}
\toprule
\textbf{Method}
& \textbf{Avg.}
& \multicolumn{2}{c}{\textbf{Main TFLOPs}}
& \multicolumn{2}{c}{\textbf{KV Cache}} \\
\cmidrule(lr){3-4}
\cmidrule(l){5-6}
& \textbf{Token}
& \textbf{Val.} & \textbf{/Vanilla}
& \textbf{MB} & \textbf{/Vanilla} \\
\midrule

\rowcolor{vanillarow}
Vanilla
& 576
& 8.38 & \na
& 342.5 & \na \\

\midrule
\rowcolor{baserow}
FastV
& 306
& 6.40 & \effdown{24}
& 213.0 & \effdown{38} \\

\rowcolor{routerow}
FastV+Reroute
& 306
& 6.53 & \effdown{22}
& 213.0 & \effdown{38} \\

\midrule
\rowcolor{baserow}
FastV
& 128
& 3.82 & \effdown{54}
& 119.2 & \effdown{65} \\

\rowcolor{routerow}
FastV+Reroute
& 128
& 3.94 & \effdown{53}
& 119.2 & \effdown{65} \\

\rowcolor{baserow}
PDrop
& 128
& 3.90 & \effdown{53}
& 117.2 & \effdown{66} \\

\rowcolor{routerow}
PDrop+Reroute
& 128
& 4.17 & \effdown{50}
& 127.6 & \effdown{63} \\

\midrule
\rowcolor{baserow}
FastV
& 64
& 2.97 & \effdown{65}
& 87.5 & \effdown{74} \\

\rowcolor{routerow}
FastV+Reroute
& 64
& 3.10 & \effdown{63}
& 87.5 & \effdown{74} \\

\rowcolor{baserow}
PDrop
& 64
& 3.33 & \effdown{60}
& 96.0 & \effdown{72} \\

\rowcolor{routerow}
PDrop+Reroute
& 64
& 3.33 & \effdown{60}
& 96.1 & \effdown{72} \\

\bottomrule
\end{tabular}

\vspace{0.25em}
{\scriptsize
\colorbox{vanillarow}{\strut Vanilla baseline}\quad
\colorbox{baserow}{\strut Base methods}\quad
\colorbox{routerow}{\strut Reroute variants}
}

\end{table}

==> tables/llava_efficiency_rot.tex <==
% ============================================================
% Required packages
% ============================================================
% \usepackage{booktabs}
% \usepackage[table]{xcolor}
% \usepackage{graphicx}
% \usepackage{array}

% ============================================================
% Macros / colors
% ============================================================
\providecommand{\na}{--}
\newcommand{\effdown}[1]{\textcolor{green!55!black}{$\downarrow$ #1\%}}
\newcommand{\effcell}[2]{#1\,{\scriptsize\effdown{#2}}}

\definecolor{vanillarow}{HTML}{EFEFEF}
\definecolor{baserow}{HTML}{FFF7E6}
\definecolor{routerow}{HTML}{EAF6EA}

% ============================================================
% Compact Efficiency Table
% ============================================================
\begin{table*}[t]
\centering
\caption{
\textbf{Efficiency comparison on LLaVA-1.5-7B under different average visual-token budgets.}
Rows denote average visual-token budgets and columns denote reduction methods.
We separately report main decoder TFLOPs and KV-cache memory; reductions are normalized against the vanilla full-token baseline.
}
\label{tab:efficiency_comparison}

\footnotesize
\setlength{\tabcolsep}{4.2pt}
\renewcommand{\arraystretch}{0.98}
\setlength{\aboverulesep}{0.22ex}
\setlength{\belowrulesep}{0.22ex}
\setlength{\cmidrulesep}{0.10ex}

\noindent
\begin{minipage}[t]{0.485\textwidth}
\centering
\textbf{(a) Main decoder TFLOPs}
\vspace{0.15em}

\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}c c c c c c@{}}
\toprule
\textbf{Avg.}
& \textbf{Vanilla}
& \textbf{FastV}
& \textbf{FastV+R}
& \textbf{PDrop}
& \textbf{PDrop+R} \\
\midrule

\rowcolor{vanillarow}
576
& 8.38
& \na
& \na
& \na
& \na \\

\midrule

306
& \na
& \cellcolor{baserow}\effcell{6.40}{24}
& \cellcolor{routerow}\effcell{6.53}{22}
& \na
& \na \\

128
& \na
& \cellcolor{baserow}\effcell{3.82}{54}
& \cellcolor{routerow}\effcell{3.94}{53}
& \cellcolor{baserow}\effcell{3.90}{53}
& \cellcolor{routerow}\effcell{4.17}{50} \\

64
& \na
& \cellcolor{baserow}\effcell{2.97}{65}
& \cellcolor{routerow}\effcell{3.10}{63}
& \cellcolor{baserow}\effcell{3.33}{60}
& \cellcolor{routerow}\effcell{3.33}{60} \\

\bottomrule
\end{tabular}%
}
\end{minipage}%
\hfill%
\begin{minipage}[t]{0.485\textwidth}
\centering
\textbf{(b) KV-cache memory (MB)}
\vspace{0.15em}

\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}c c c c c c@{}}
\toprule
\textbf{Avg.}
& \textbf{Vanilla}
& \textbf{FastV}
& \textbf{FastV+R}
& \textbf{PDrop}
& \textbf{PDrop+R} \\
\midrule

\rowcolor{vanillarow}
576
& 342.5
& \na
& \na
& \na
& \na \\

\midrule

306
& \na
& \cellcolor{baserow}\effcell{213.0}{38}
& \cellcolor{routerow}\effcell{213.0}{38}
& \na
& \na \\

128
& \na
& \cellcolor{baserow}\effcell{119.2}{65}
& \cellcolor{routerow}\effcell{119.2}{65}
& \cellcolor{baserow}\effcell{117.2}{66}
& \cellcolor{routerow}\effcell{127.6}{63} \\

64
& \na
& \cellcolor{baserow}\effcell{87.5}{74}
& \cellcolor{routerow}\effcell{87.5}{74}
& \cellcolor{baserow}\effcell{96.0}{72}
& \cellcolor{routerow}\effcell{96.1}{72} \\

\bottomrule
\end{tabular}%
}
\end{minipage}

\vspace{0.25em}
{\scriptsize
\colorbox{vanillarow}{\strut Vanilla baseline}\quad
\colorbox{baserow}{\strut Base methods}\quad
\colorbox{routerow}{\strut Reroute variants}
}

\end{table*}

==> tables/llava_vg.tex <==
% Required packages:
% \usepackage{booktabs}
% \usepackage[table]{xcolor}
% \usepackage{graphicx}

\begin{table}[t]
\centering
\caption{
Performance comparison on RefCOCO-series visual grounding benchmarks using
LLaVA-1.5-7B. Best and second-best results within each average-token block are
shown in \best{bold} and \second{underlined}, respectively.
}
\label{tab:llava15_refcoco_main}
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.08}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}llccccccccc@{}}
\toprule
\textbf{Method} & \textbf{Source}
& \multicolumn{3}{c}{\textbf{RefCOCO}}
& \multicolumn{3}{c}{\textbf{RefCOCO+}}
& \multicolumn{2}{c}{\textbf{RefCOCOg}}
& \shortstack[c]{\textbf{Avg.}} \\
\cmidrule(lr){3-5}
\cmidrule(lr){6-8}
\cmidrule(lr){9-10}
& & \textbf{val} & \textbf{A} & \textbf{B}
& \textbf{val} & \textbf{A} & \textbf{B}
& \textbf{val} & \textbf{test}
& \textbf{Ratio}\\
\midrule

\multicolumn{11}{c}{\textit{Average Token 576}} \\
\midrule
\rowcolor{vanillarow}
Vanilla\Oformat
& CVPR'24
& \best{56.4} & \na & \na
& 46.3 & \best{59.4} & \second{38.9}
& \best{48.8} & \best{48.5}
& \best{100.0\%} \\

\rowcolor{vanillarow}
Vanilla\Oformat\Repro
& CVPR'24
& \second{56.2} & \best{64.6} & \second{47.6}
& \best{50.0} & \second{59.3} & 38.8
& \best{48.8} & \second{48.4}
& \best{100.0\%} \\

\rowcolor{vanillarow}
Vanilla\HFformat
& CVPR'24
& 54.0 & \second{59.4} & \best{48.0}
& \second{46.5} & 54.1 & \best{39.1}
& \second{46.9} & 47.6
& \best{100.0\%} \\

\midrule
\multicolumn{11}{c}{\textit{Average Token 192} $\downarrow 66.7\%$} \\
\midrule
\rowcolor{otherrow}
FEATHER\Oformat
& ICCV'25
& \na & \na & \na
& \na & 24.7 & \na
& \na & 27.2
& 48.8\% \\

\midrule
\rowcolor{baserow}
FastV\HFformat\Repro
& ECCV'24
& 25.3 & 27.8 & 22.3
& 21.0 & 23.6 & 18.0
& 21.5 & 20.5
& 45.5\% \\

\rowcolor{baserow}
PDrop\HFformat\Repro
& CVPR'25
& 39.8 & 45.1 & 33.4
& 33.5 & 39.5 & 25.9
& 33.2 & 32.8
& 71.3\% \\

\rowcolor{baserow}
N\"uwa\Oformat
& ICLR'26
& 46.1 & \na & \na
& 37.7 & 43.2 & 31.9
& 37.9 & 37.6
& 78.8\% \\

\rowcolor{baserow}
N\"uwa\Oformat\Repro
& ICLR'26
& \best{59.1} & \second{67.5} & \best{48.9}
& \best{50.5} & \second{60.9} & \best{40.2}
& \best{51.8} & \best{50.1}
& \best{103.7\%} \\

\midrule
\rowcolor{routerow}
FastV+Reroute\HFformat
& Ours
& 32.7 & 37.7 & 26.8
& 26.7 & 32.3 & 21.3
& 28.7 & 29.1
& 59.2\% \\

\rowcolor{routerow}
PDrop+Reroute\HFformat
& Ours
& 45.3 & 49.5 & 39.0
& 37.9 & 44.3 & 31.1
& 39.7 & 39.2
& 82.3\% \\

\rowcolor{routerow}
N\"uwa+Reroute\Oformat
& Ours
& \second{58.6} & \best{67.8} & \second{48.7}
& \second{50.4} & \best{61.3} & \second{39.8}
& \second{50.9} & \second{49.9}
& \second{103.2\%} \\

\midrule
\multicolumn{11}{c}{\textit{Average Token 128} $\downarrow 77.8\%$} \\
\midrule
\rowcolor{otherrow}
SparseVLM\Oformat
& ICML'25
& 6.2 & \na & \na
& 9.9 & 5.8 & 4.2
& 6.5 & 6.4
& 13.2\% \\

\rowcolor{otherrow}
VisionZip\Oformat
& CVPR'25
& 4.1 & \na & \na
& 3.9 & 4.1 & 4.9
& 3.5 & 3.5
& 8.3\% \\

\midrule
\rowcolor{baserow}
FastV\HFformat\Repro
& ECCV'24
& 11.0 & 12.7 & 9.1
& 8.9 & 10.3 & 8.0
& 9.3 & 9.0
& 19.8\% \\

\rowcolor{baserow}
PDrop\HFformat\Repro
& CVPR'25
& 30.7 & 36.5 & 23.7
& 25.2 & 30.5 & 18.3
& 24.4 & 23.9
& 53.4\% \\

\rowcolor{baserow}
N\"uwa\Oformat
& ICLR'26
& 43.7 & \na & \na
& 35.3 & 42.6 & 29.0
& 36.0 & 36.6
& 74.9\% \\

\rowcolor{baserow}
N\"uwa\Oformat\Repro
& ICLR'26
& \best{52.3} & \best{61.4} & \best{42.9}
& \second{43.7} & \second{53.2} & \best{35.6}
& \best{45.0} & \best{43.5}
& \best{91.1\%} \\

\midrule
\rowcolor{routerow}
FastV+Reroute\HFformat
& Ours
& 17.4 & 20.7 & 13.9
& 14.5 & 17.5 & 11.6
& 15.8 & 15.1
& 31.8\% \\

\rowcolor{routerow}
PDrop+Reroute\HFformat
& Ours
& 34.1 & 39.6 & 27.2
& 27.6 & 33.2 & 22.0
& 29.8 & 29.7
& 61.2\% \\

\rowcolor{routerow}
N\"uwa+Reroute\Oformat
& Ours
& \second{51.8} & \best{61.4} & \second{42.6}
& \best{44.3} & \best{53.5} & \second{35.0}
& \second{44.3} & \second{43.1}
& \second{90.7\%} \\

\midrule
\multicolumn{11}{c}{\textit{Average Token 64} $\downarrow 88.9\%$} \\
\midrule
\rowcolor{otherrow}
SparseVLM\Oformat
& ICML'25
& 1.0 & \na & \na
& 1.0 & 1.0 & 1.3
& 0.7 & 0.6
& 1.9\% \\

\rowcolor{otherrow}
VisionZip\Oformat
& CVPR'25
& 3.8 & \na & \na
& 3.5 & 3.7 & 3.9
& 3.2 & 3.4
& 7.4\% \\

\midrule
\rowcolor{baserow}
FastV\HFformat\Repro
& ECCV'24
& 0.3 & 0.2 & 0.6
& 0.3 & 0.1 & 0.5
& 0.1 & 0.1
& 0.6\% \\

\rowcolor{baserow}
PDrop\HFformat\Repro
& CVPR'25
& 12.8 & 14.8 & 10.2
& 10.1 & 12.1 & 8.0
& 10.3 & 10.1
& 22.2\% \\

\rowcolor{baserow}
N\"uwa\Oformat
& ICLR'26
& \second{28.6} & \na & \na
& 22.2 & 28.2 & 17.5
& 21.4 & 21.8
& 46.7\% \\

\rowcolor{baserow}
N\"uwa\Oformat\Repro
& ICLR'26
& \best{32.8} & \best{40.6} & \second{24.5}
& \second{26.5} & \second{34.3} & \second{20.5}
& \second{25.6} & \second{24.5}
& \second{54.9\%} \\

\midrule
\rowcolor{routerow}
FastV+Reroute\HFformat
& Ours
& 0.4 & 0.2 & 0.4
& 0.3 & 0.1 & 0.7
& 0.1 & 0.1
& 0.6\% \\

\rowcolor{routerow}
PDrop+Reroute\HFformat
& Ours
& 18.9 & 23.3 & 14.5
& 15.4 & 19.9 & 11.5
& 16.5 & 15.6
& 34.0\% \\

\rowcolor{routerow}
N\"uwa+Reroute\Oformat
& Ours
& \best{32.8} & \second{40.5} & \best{24.9}
& \best{27.2} & \best{35.3} & \best{21.1}
& \best{26.3} & \best{25.2}
& \best{56.0\%} \\

\bottomrule
\end{tabular}%
}

\vspace{0.35em}
\footnotesize{
\colorbox{vanillarow}{Vanilla baseline};
\colorbox{otherrow}{Other methods};
\colorbox{baserow}{Base methods};
\colorbox{routerow}{Reroute variants}. \\
\Oformat: original LLaVA / haotian-liu format;
\HFformat: HuggingFace-format model;
\Repro: reproduced result;
: reroute variant.
Unavailable results are denoted by ``--''.
For RefCOCO and RefCOCO+, A/B denote testA/testB.
Avg. Ratio is the mean score ratio against the corresponding vanilla baseline,
computed over subsets where both scores are available.
Schedule details are reported in the appendix.
}
\end{table}

==> tables/llava_vg_paper.tex <==
% Required packages:
% \usepackage{booktabs}
% \usepackage[table]{xcolor}
% \usepackage{graphicx}

% ============================================================
% Table 1: Original LLaVA / Nuwa official-codebase format
% ============================================================
\begin{table}[t]
\centering
\caption{
\textbf{Visual grounding performance comparison on RefCOCO-series benchmarks using
LLaVA-1.5-7B under the original LLaVA / Nuwa official-codebase format.}
Prior-method rows are paper-reported results, while rows marked with
\NuwaOfficial{} are reproduced in the official N\"uwa codebase.
Best and second-best results within each average-token block are shown in
\best{bold} and \second{underlined}, respectively.
}
\label{tab:llava15_refcoco_original_format}
\small
% \setlength{\tabcolsep}{3.2pt}
% \renewcommand{\arraystretch}{1.08}
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}llcccccccc@{}}
\toprule
\textbf{Method} & \textbf{Source}
& \multicolumn{2}{c}{\textbf{RefCOCO}}
& \multicolumn{3}{c}{\textbf{RefCOCO+}}
& \multicolumn{2}{c}{\textbf{RefCOCOg}}
& \shortstack[c]{\textbf{Avg.}} \\
\cmidrule(lr){3-4}
\cmidrule(lr){5-7}
\cmidrule(lr){8-9}
& & \textbf{val} & \textbf{test}
& \textbf{val} & \textbf{A} & \textbf{B}
& \textbf{val} & \textbf{test}
& \textbf{Ratio} \\
\midrule

\multicolumn{10}{c}{\textit{Average Token 576}} \\
\midrule

\rowcolor{vanillarow}
Vanilla\NuwaOfficial
& CVPR'24
& \best{56.2} & \best{58.0}
& \best{50.0} & \best{59.3} & \best{38.8}
& \best{48.9} & \best{48.4}
& \best{100.0\%} \\

\midrule
\multicolumn{10}{c}{\textit{Average Token 192} $\downarrow 66.7\%$} \\
\midrule

\rowcolor{otherrow}
FEATHER
& ICCV'25
& \na & 27.7
& \na & 2.5 & \na
& \na & 27.2
& 36.1\% \\

\midrule

\rowcolor{baserow}
N\"uwa\NuwaOfficial
& ICLR'26
& \best{59.1} & \best{60.1}
& \best{50.5} & \second{60.9} & \best{40.2}
& \best{51.8} & \best{50.1}
& \best{103.7\%} \\

\rowcolor{routerow}
N\"uwa+Reroute\NuwaOfficial
& Ours
& \second{58.6} & \second{59.6}
& \second{50.4} & \best{61.3} & \second{39.8}
& \second{50.9} & \second{49.9}
& \second{103.0\%} \\

\midrule
\multicolumn{10}{c}{\textit{Average Token 128} $\downarrow 77.8\%$} \\
\midrule

\rowcolor{otherrow}
FastV
& ECCV'24
& 10.1 & 10.3
& 8.2 & 8.5 & 9.8
& 9.1 & 8.9
& 18.4\% \\

\rowcolor{otherrow}
SparseVLM
& ICML'25
& 6.2 & 6.3
& 9.9 & 5.8 & 4.2
& 6.5 & 6.4
& 12.6\% \\

\rowcolor{otherrow}
VisionZip
& CVPR'25
& 4.1 & 4.5
& 3.9 & 4.1 & 4.9
& 3.5 & 3.5
& 8.1\% \\

\midrule

\rowcolor{baserow}
N\"uwa\NuwaOfficial
& ICLR'26
& \best{52.3} & \best{53.5}
& \second{43.7} & \second{53.2} & \best{35.6}
& \best{45.0} & \best{43.5}
& \best{90.9\%} \\

\rowcolor{routerow}
N\"uwa+Reroute\NuwaOfficial
& Ours
& \second{51.8} & \second{53.0}
& \best{44.3} & \best{55.5} & \second{35.0}
& \second{44.3} & \second{43.1}
& \second{90.3\%} \\

\midrule
\multicolumn{10}{c}{\textit{Average Token 64} $\downarrow 88.9\%$} \\
\midrule

\rowcolor{otherrow}
FastV
& ECCV'24
& 2.0 & 2.7
& 2.4 & 1.2 & 1.0
& 2.0 & 2.2
& 3.8\% \\

\rowcolor{otherrow}
SparseVLM
& ICML'25
& 1.0 & 1.0
& 1.0 & 1.0 & 1.3
& 0.7 & 0.6
& 1.9\% \\

\rowcolor{otherrow}
VisionZip
& CVPR'25
& 3.8 & 4.0
& 3.5 & 3.7 & 3.9
& 3.2 & 3.4
& 7.2\% \\

\midrule

\rowcolor{baserow}
N\"uwa\NuwaOfficial
& ICLR'26
& \best{32.8} & \second{33.2}
& \second{26.5} & \second{34.3} & \second{20.5}
& \second{25.6} & \second{24.5}
& \second{54.6\%} \\

\rowcolor{routerow}
N\"uwa+Reroute\NuwaOfficial
& Ours
& \best{32.8} & \best{33.7}
& \best{27.2} & \best{35.3} & \best{21.1}
& \best{26.3} & \best{25.2}
& \best{55.8\%} \\

\bottomrule
\end{tabular}%
% }

\vspace{0.35em}
\footnotesize{
\colorbox{vanillarow}{Vanilla baseline};
\colorbox{otherrow}{Other methods};
\colorbox{baserow}{Base methods};
\colorbox{routerow}{Reroute variants}. \\
\NuwaOfficial{}: reproduced in the official N\"uwa codebase.
Unavailable results are denoted by ``--''.
For RefCOCO+, A/B denote testA/testB.
Avg. Ratio is reported relative to the corresponding full-token baseline.
}
\end{table}

==> tables/llava_vg_repr.tex <==
% ============================================================
% Table 2: HuggingFace-format reproduced visual grounding results
% ============================================================
\begin{table}[t]
\centering
\caption{
\textbf{Reproduced visual grounding performance comparison on RefCOCO-series benchmarks
using the HuggingFace-format LLaVA-1.5-7B checkpoint.} All rows are evaluated in
our unified pipeline, so numbers are intended for within-table comparison rather
than direct comparison with original-format paper-reported results.
Best and second-best results within each average-token block are shown in
\best{bold} and \second{underlined}, respectively.
}
\label{tab:llava15_refcoco_hf_format}
\small
% \setlength{\tabcolsep}{2.9pt}
% \renewcommand{\arraystretch}{1.08}
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}llccccccccc@{}}
\toprule
\textbf{Method} & \textbf{Source}
& \multicolumn{3}{c}{\textbf{RefCOCO}}
& \multicolumn{3}{c}{\textbf{RefCOCO+}}
& \multicolumn{2}{c}{\textbf{RefCOCOg}}
& \shortstack[c]{\textbf{Avg.}} \\
\cmidrule(lr){3-5}
\cmidrule(lr){6-8}
\cmidrule(lr){9-10}
& & \textbf{val} & \textbf{A} & \textbf{B}
& \textbf{val} & \textbf{A} & \textbf{B}
& \textbf{val} & \textbf{test}
& \textbf{Ratio} \\
\midrule

\multicolumn{11}{c}{\textit{Average Token 576}} \\
\midrule

\rowcolor{vanillarow}
Vanilla HF
& CVPR'24
& \best{54.0} & \best{59.4} & \best{48.0}
& \best{46.5} & \best{54.1} & \best{39.1}
& \best{46.9} & \best{47.6}
& \best{100.0\%} \\

\midrule
\multicolumn{11}{c}{\textit{Average Token 192} $\downarrow 66.7\%$} \\
\midrule

\rowcolor{baserow}
FastV
& ECCV'24
& 25.3 & 27.8 & 22.3
& 21.0 & 23.6 & 18.0
& 21.5 & 20.5
& 45.5\% \\

\rowcolor{routerow}
FastV+Reroute
& Ours
& 32.7 & 37.7 & 26.8
& 26.7 & 32.3 & 21.3
& 28.7 & 29.1
& 59.2\% \\

\rowcolor{baserow}
PDrop
& CVPR'25
& \second{39.8} & \second{45.1} & \second{33.4}
& \second{33.5} & \second{39.5} & \second{25.9}
& \second{33.2} & \second{32.8}
& \second{71.3\%} \\

\rowcolor{routerow}
PDrop+Reroute
& Ours
& \best{45.3} & \best{49.5} & \best{39.0}
& \best{37.9} & \best{44.3} & \best{31.1}
& \best{39.7} & \best{39.2}
& \best{82.3\%} \\

\midrule
\multicolumn{11}{c}{\textit{Average Token 128} $\downarrow 77.8\%$} \\
\midrule

\rowcolor{baserow}
FastV
& ECCV'24
& 11.0 & 12.7 & 9.1
& 8.9 & 10.3 & 8.0
& 9.3 & 9.0
& 19.8\% \\

\rowcolor{routerow}
FastV+Reroute
& Ours
& 17.4 & 20.7 & 13.9
& 14.5 & 17.5 & 11.6
& 15.8 & 15.1
& 31.8\% \\

\rowcolor{baserow}
PDrop
& CVPR'25
& \second{30.7} & \second{36.5} & \second{23.7}
& \second{25.2} & \second{30.5} & \second{18.3}
& \second{24.4} & \second{23.9}
& \second{53.4\%} \\

\rowcolor{routerow}
PDrop+Reroute
& Ours
& \best{34.1} & \best{39.6} & \best{27.2}
& \best{27.6} & \best{33.2} & \best{22.0}
& \best{29.8} & \best{29.7}
& \best{61.2\%} \\

\midrule
\multicolumn{11}{c}{\textit{Average Token 64} $\downarrow 88.9\%$} \\
\midrule

\rowcolor{baserow}
FastV
& ECCV'24
& 0.3 & 0.2 & 0.6
& 0.3 & 0.1 & 0.5
& 0.1 & 0.1
& 0.6\% \\

\rowcolor{routerow}
FastV+Reroute
& Ours
& 0.4 & 0.2 & 0.4
& 0.3 & 0.1 & 0.7
& 0.1 & 0.1
& 0.6\% \\

\rowcolor{baserow}
PDrop
& CVPR'25
& \second{12.8} & \second{14.8} & \second{10.2}
& \second{10.1} & \second{12.1} & \second{8.0}
& \second{10.3} & \second{10.1}
& \second{22.2\%} \\

\rowcolor{routerow}
PDrop+Reroute
& Ours
& \best{18.9} & \best{23.3} & \best{14.5}
& \best{15.4} & \best{19.9} & \best{11.5}
& \best{16.5} & \best{15.6}
& \best{34.0\%} \\

\bottomrule
\end{tabular}%
% }

\vspace{0.35em}
\footnotesize{
\colorbox{vanillarow}{Vanilla baseline};
\colorbox{baserow}{Base methods};
\colorbox{routerow}{Reroute variants}. \\
All rows are reproduced under the HuggingFace-format model in our unified pipeline.
For RefCOCO and RefCOCO+, A/B denote testA/testB.
Avg. Ratio is normalized by the HF-format full-token baseline.
}
\end{table}

==> tables/llava_vqa.tex <==
% Required packages:
% \usepackage{booktabs}
% \usepackage[table]{xcolor}
% \usepackage{graphicx}
% \usepackage{tabularx}
% \usepackage{array}


% ============================================================
% VQA Table
% ============================================================

\begin{table*}[t]
\centering
\caption{
VQA performance comparison on LLaVA-1.5-7B.
Best and second-best results within each average-token block are shown in
\best{bold} and \second{underlined}, respectively.
}
\label{tab:llava15_vqa_main}
\scriptsize
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.08}
\resizebox{\linewidth}{!}{%
\begin{tabular}{llcccccccccc}
\toprule
\textbf{Method} & \textbf{Source}
& \textbf{GQA} & \textbf{MMB} & \textbf{MMMU} & \textbf{MME}
& \textbf{VQAv2} & \textbf{TextVQA} & \textbf{POPE} & \textbf{SQA} & \textbf{SEED}
& \textbf{Avg. Ratio} \\
\midrule

\multicolumn{12}{c}{\textit{Average Token 576}} \\
\midrule
\rowcolor{vanillarow}
Vanilla\Oformat
& CVPR'24
& \best{61.9} & \best{64.7} & \best{36.3} & \best{1862}
& \best{78.5} & \best{58.2} & \best{85.9} & \best{69.5} & \second{58.6}
& \best{100.0\%} \\

\rowcolor{vanillarow}
Vanilla\HFformat\Repro
& CVPR'24
& \second{60.5} & \second{62.4} & \second{34.4} & \second{1782}
& \second{69.8} & \second{57.5} & \best{85.9} & \second{66.1} & \best{65.5}
& \best{100.0\%} \\

\midrule
\multicolumn{12}{c}{\textit{Average Token 192} $\downarrow 66.7\%$} \\
\midrule
\rowcolor{otherrow}
SparseVLM\Oformat
& ICML'25
& 57.6 & 62.5 & 33.8 & 1721
& 75.6 & 56.1 & 83.6 & \best{69.1} & 55.8
& 95.5\% \\

\rowcolor{otherrow}
VisionZip\Oformat
& CVPR'25
& 59.3 & 63.0 & \best{36.6} & 1782
& \best{76.8} & 57.3 & 85.3 & \second{68.9} & 56.4
& 97.9\% \\

\addlinespace[1pt]
\rowcolor{baserow}
FastV\HFformat\Repro
& ECCV'24
& 55.0 & 58.6 & 34.2 & 1637
& 63.2 & 53.7 & 79.6 & 66.4 & 58.2
& 93.6\% \\

\rowcolor{baserow}
PDrop\HFformat\Repro
& CVPR'25
& 59.2 & 61.4 & 34.7 & 1776
& 68.7 & 46.9 & 84.4 & 65.9 & \second{63.4}
& 96.8\% \\

\rowcolor{baserow}
N\"uwa\Oformat
& ICLR'26
& \second{60.9} & \best{64.3} & 35.5 & \second{1834}
& \second{75.9} & \second{57.4} & \best{86.4} & 68.2 & 59.7
& \second{98.9\%} \\

\addlinespace[1pt]
\rowcolor{routerow}
FastV+Reroute\HFformat\Route
& Ours
& 57.4 & 60.7 & 34.2 & 1672
& 66.4 & 56.7 & 81.0 & 67.1 & 60.4
& 96.4\% \\

\rowcolor{routerow}
PDrop+Reroute\HFformat\Route
& Ours
& 58.9 & 61.3 & 34.4 & 1775
& 68.4 & \second{57.4} & 84.2 & 66.1 & 62.6
& 98.5\% \\

\rowcolor{routerow}
N\"uwa+Reroute\Oformat\Route
& Ours
& \best{61.1} & \second{63.6} & \second{35.7} & \best{1848}
& \na & \best{57.8} & \second{86.0} & \na & \best{66.1}
& \best{101.0\%} \\

\midrule
\multicolumn{12}{c}{\textit{Average Token 128} $\downarrow 77.8\%$} \\
\midrule
\rowcolor{otherrow}
SparseVLM\Oformat
& ICML'25
& 56.0 & 60.0 & 33.8 & 1696
& 73.8 & 54.9 & 80.5 & 67.1 & 53.4
& 93.0\% \\

\rowcolor{otherrow}
VisionZip\Oformat
& CVPR'25
& 57.6 & 62.0 & \best{37.9} & 1761
& \best{75.6} & 56.8 & 83.2 & \best{68.9} & 54.9
& 96.8\% \\

\rowcolor{otherrow}
PruMerge\Oformat
& ICCV'25
& 57.8 & 59.6 & \second{36.2} & 1712
& 74.7 & 54.3 & 81.5 & 67.6 & \na
& 94.7\% \\

\addlinespace[1pt]
\rowcolor{baserow}
FastV\HFformat\Repro
& ECCV'24
& 50.5 & 53.7 & 34.0 & 1451
& 56.2 & 50.4 & 73.0 & 65.5 & 54.3
& 87.2\% \\

\rowcolor{baserow}
PDrop\HFformat\Repro
& CVPR'25
& 57.0 & 59.5 & 34.2 & 1728
& 66.3 & 56.2 & 82.1 & 66.8 & 59.2
& 96.2\% \\

\rowcolor{baserow}
N\"uwa\Oformat
& ICLR'26
& \second{60.2} & \best{63.4} & 35.8 & \best{1828}
& \second{75.1} & \second{57.0} & \best{85.5} & 67.8 & 58.7
& \second{98.1\%} \\

\addlinespace[1pt]
\rowcolor{routerow}
FastV+Reroute\HFformat\Route
& Ours
& 54.8 & 57.0 & 34.3 & 1557
& 62.0 & 53.6 & 75.1 & \second{68.4} & 55.4
& 91.8\% \\

\rowcolor{routerow}
PDrop+Reroute\HFformat\Route
& Ours
& 57.3 & 59.8 & 34.6 & 1733
& 65.7 & 56.5 & 80.9 & 66.6 & \second{60.8}
& 96.5\% \\

\rowcolor{routerow}
N\"uwa+Reroute\Oformat\Route
& Ours
& \best{60.4} & \second{63.2} & 36.1 & \second{1827}
& \na & \best{57.3} & \second{85.3} & \na & \best{64.4}
& \best{100.1\%} \\

\midrule
\multicolumn{12}{c}{\textit{Average Token 64} $\downarrow 88.9\%$} \\
\midrule
\rowcolor{otherrow}
SparseVLM\Oformat
& ICML'25
& 53.8 & 60.1 & 35.4 & 1589
& 68.2 & 53.4 & 77.5 & \best{69.8} & 51.1
& 91.0\% \\

\rowcolor{otherrow}
VisionZip\Oformat
& CVPR'25
& 55.1 & 60.1 & \second{36.2} & \second{1690}
& \second{72.4} & \best{55.5} & 77.0 & 69.0 & 52.2
& 93.1\% \\

\rowcolor{otherrow}
PruMerge\Oformat
& ICCV'25
& 55.4 & 59.6 & 35.8 & 1616
& 71.3 & 52.0 & 75.7 & \second{69.5} & \na
& 91.9\% \\

\addlinespace[1pt]
\rowcolor{baserow}
FastV\HFformat\Repro
& ECCV'24
& 40.0 & 22.4 & 32.1 & 950
& 39.2 & 41.8 & 51.1 & 65.1 & 36.0
& 65.6\% \\

\rowcolor{baserow}
PDrop\HFformat\Repro
& CVPR'25
& 52.8 & 55.1 & 33.1 & 1486
& 60.6 & 51.6 & 74.9 & 68.2 & 53.9
& 89.4\% \\

\rowcolor{baserow}
N\"uwa\Oformat
& ICLR'26
& \second{58.3} & \best{62.0} & \best{36.4} & \best{1706}
& \best{72.8} & 54.9 & \best{83.0} & 67.5 & \second{56.4}
& \second{95.4\%} \\

\addlinespace[1pt]
\rowcolor{routerow}
FastV+Reroute\HFformat\Route
& Ours
& 44.3 & 23.3 & 32.2 & 954
& 44.6 & 43.5 & 51.4 & 65.3 & 39.8
& 68.5\% \\

\rowcolor{routerow}
PDrop+Reroute\HFformat\Route
& Ours
& 54.4 & 57.4 & 33.8 & 1542
& 61.7 & 52.5 & 74.8 & 69.2 & 54.8
& 91.3\% \\

\rowcolor{routerow}
N\"uwa+Reroute\Oformat\Route
& Ours
& \best{58.5} & \second{61.9} & 35.9 & 1688
& \na & \second{55.1} & \second{82.6} & \na & \best{61.6}
& \best{96.5\%} \\

\bottomrule
\end{tabular}%
}
\vspace{0.3em}
\footnotesize{
\colorbox{vanillarow}{Vanilla baseline};
\colorbox{otherrow}{Other methods};
\colorbox{baserow}{Base methods};
\colorbox{routerow}{Reroute variants}.
\Oformat: original LLaVA / haotian-liu format;
\HFformat: HuggingFace-format model;
\Repro: reproduced run;
\Route: reroute variant.
Unavailable results are denoted by ``--''.
Avg. Ratio is the mean score ratio against the corresponding vanilla baseline,
computed over subsets where both scores are available.
Schedule details are omitted here and reported in the appendix.
}
\end{table*}

==> tables/llava_vqa_repr.tex <==
% ============================================================
% Table 2: HuggingFace-format reproduced VQA results
% ============================================================
\begin{table*}[t]
\centering
\caption{
Reproduced VQA performance comparison on LLaVA-1.5-7B under the HuggingFace
model format. All rows are evaluated in our unified pipeline using the
HF-format LLaVA-1.5-7B checkpoint. Only tasks available in the updated result
sheet are reported. Best and second-best results within each average-token block
are shown in \best{bold} and \second{underlined}, respectively.
}
\label{tab:llava15_vqa_hf_format}
\scriptsize
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.08}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}llccccccccc@{}}
\toprule
\textbf{Method} & \textbf{Source}
& \textbf{GQA} & \textbf{MMB} & \textbf{MMMU} & \textbf{MME}
& \textbf{TextVQA} & \textbf{POPE} & \textbf{SQA}
& \textbf{SEED} & \textbf{Avg. Ratio} \\
\midrule

\multicolumn{11}{c}{\textit{Average Token 576}} \\
\midrule

\rowcolor{vanillarow}
Baseline
& CVPR'24
& \best{60.5} & \best{62.4} & \best{34.4} & \best{1782}
& \best{57.5} & \best{85.9} & \best{66.1}
& \best{65.5} & \best{100.0\%} \\

\midrule
\multicolumn{11}{c}{\textit{Average Token 192} $\downarrow 66.7\%$} \\
\midrule

\rowcolor{baserow}
FastV (L3)
& ECCV'24
& 55.0 & 58.6 & 34.2 & 1637
& 53.7 & 79.6 & 66.4
& 58.2 & 93.9\% \\

\rowcolor{routerow}
FastV+Reroute
& Ours
& 57.4 & 60.7 & 34.2 & 1672
& \second{56.7} & 81.0 & \second{67.1}
& 60.4 & 96.5\% \\

\rowcolor{baserow}
PDrop (L8)
& CVPR'25
& 56.4 & 58.9 & \second{34.4} & 1685
& 55.1 & 81.0 & \best{68.4}
& 58.4 & 95.6\% \\

\rowcolor{baserow}
PDrop (L2)
& CVPR'25
& \best{59.2} & \best{61.4} & \best{34.7} & \best{1776}
& 46.9 & \best{84.4} & 65.9
& \best{63.4} & \second{96.6\%} \\

\rowcolor{routerow}
PDrop+Reroute
& Ours
& \second{58.9} & \second{61.3} & \second{34.4} & \second{1775}
& \best{57.4} & \second{84.2} & 66.1
& \second{62.6} & \best{98.6\%} \\

\midrule
\multicolumn{11}{c}{\textit{Average Token 128} $\downarrow 77.8\%$} \\
\midrule

\rowcolor{baserow}
FastV (L3)
& ECCV'24
& 50.5 & 53.7 & 34.0 & 1451
& 50.4 & 73.0 & 65.5
& 54.3 & 88.0\% \\

\rowcolor{baserow}
PDrop (L2)
& CVPR'25
& \second{57.0} & \second{59.5} & 34.2 & \second{1728}
& \second{56.2} & \best{82.1} & \second{66.8}
& \second{59.2} & \second{96.3\%} \\

\rowcolor{routerow}
FastV+Reroute
& Ours
& 54.8 & 57.0 & \second{34.3} & 1557
& 53.6 & 75.1 & \best{68.4}
& 55.4 & 92.2\% \\

\rowcolor{routerow}
PDrop+Reroute
& Ours
& \best{57.3} & \best{59.8} & \best{34.6} & \best{1733}
& \best{56.5} & \second{80.9} & 66.6
& \best{60.8} & \best{96.8\%} \\

\midrule
\multicolumn{11}{c}{\textit{Average Token 64} $\downarrow 88.9\%$} \\
\midrule

\rowcolor{baserow}
FastV
& ECCV'24
& 40.0 & 22.4 & 32.1 & 950
& 41.8 & 51.1 & 65.1
& 36.0 & 66.8\% \\

\rowcolor{baserow}
PDrop
& CVPR'25
& \second{52.8} & \second{55.1} & \second{33.1} & \second{1486}
& \second{51.6} & \best{74.9} & \second{68.2}
& \second{53.9} & \second{89.7\%} \\

\rowcolor{routerow}
FastV+Reroute
& Ours
& 44.3 & 23.3 & 32.2 & 954
& 43.5 & 51.4 & 65.3
& 39.8 & 69.1\% \\

\rowcolor{routerow}
PDrop+Reroute
& Ours
& \best{54.4} & \best{57.4} & \best{33.8} & \best{1542}
& \best{52.5} & \second{74.8} & \best{69.2}
& \best{54.8} & \best{91.7\%} \\

\bottomrule
\end{tabular}%
}

\vspace{0.35em}
\footnotesize{
\colorbox{vanillarow}{Vanilla baseline};
\colorbox{baserow}{Base methods};
\colorbox{routerow}{Reroute variants}. \\
All rows are reproduced under the HuggingFace-format model in our unified pipeline.
MMB denotes MMBench; SQA denotes ScienceQA; SEED denotes SeedBench.
Avg. Ratio is normalized by the HF-format full-token baseline.
}
\end{table*}

==> tables/qwen25vl_vg.tex <==
% Required packages:
% \usepackage{booktabs}
% \usepackage[table]{xcolor}
% \usepackage{graphicx}


% ============================================================
% Qwen2.5-VL Visual Grounding / RefCOCO Table
% ============================================================

\begin{table}[t]
\centering
\caption{
\textbf{Performance comparison on RefCOCO-series visual grounding benchmarks using
Qwen2.5-VL-7B.} Best and second-best results within each average-token block are
shown in \best{bold} and \second{underlined}, respectively.
}
\label{tab:qwen25vl_refcoco_main}
\small
% \setlength{\tabcolsep}{3.0pt}
% \renewcommand{\arraystretch}{1.08}
% \resizebox{\linewidth}{!}{%
{
\begin{tabular}{@{}llccccccccc@{}}
\toprule
\textbf{Method} & \textbf{Source}
& \multicolumn{3}{c}{\textbf{RefCOCO}}
& \multicolumn{3}{c}{\textbf{RefCOCO+}}
& \multicolumn{2}{c}{\textbf{RefCOCOg}}
& \shortstack[c]{\textbf{Avg.}} \\
\cmidrule(lr){3-5}
\cmidrule(lr){6-8}
\cmidrule(lr){9-10}
& & \textbf{val} & \textbf{A} & \textbf{B}
& \textbf{val} & \textbf{A} & \textbf{B}
& \textbf{val} & \textbf{test}
& \textbf{Ratio}\\
\midrule

\multicolumn{11}{c}{\textit{Average Token (100\%)}} \\
\midrule
\rowcolor{vanillarow}
Vanilla
& Qwen'25
& \best{87.7} & \best{89.8} & \best{82.3}
& \best{80.5} & \best{85.9} & \best{72.8}
& \best{82.7} & \best{83.3}
& \best{100.0\%} \\

\midrule
\multicolumn{11}{c}{\textit{Average Token Reduction} $\downarrow 66.7\%$} \\
\midrule
\rowcolor{baserow}
FastV
& ECCV'24
& 46.4 & 48.1 & 44.4
& 40.5 & 42.6 & 39.3
& 48.4 & 47.2
& 53.7\% \\

\rowcolor{baserow}
PDrop(L8)
& CVPR'25
& 33.4 & 39.3 & 28.5
& 28.9 & 34.6 & 23.3
& 32.7 & 33.1
& 38.0\% \\

\rowcolor{baserow}
PDrop(L2)
& CVPR'25
& \second{55.9} & \second{59.2} & \second{52.0}
& \second{48.4} & \second{53.0} & \second{43.6}
& \second{53.6} & \second{52.9}
& \second{62.9\%} \\

\midrule
\rowcolor{routerow}
FastV+Reroute\Route
& Ours
& 53.4 & 57.8 & 49.4
& 45.0 & 50.9 & 40.6
& 52.8 & 52.1
& 60.3\% \\

\rowcolor{routerow}
PDrop+Reroute\Route
& Ours
& \best{57.9} & \best{63.0} & \best{53.6}
& \best{49.9} & \best{55.7} & \best{44.8}
& \best{54.7} & \best{54.0}
& \best{65.1\%} \\

\midrule
\multicolumn{11}{c}{\textit{Average Token Reduction} $\downarrow 77.8\%$} \\
\midrule
\rowcolor{baserow}
FastV
& ECCV'24
& 19.2 & 21.5 & 17.8
& 16.7 & 18.4 & 14.6
& 19.1 & 18.6
& 21.9\% \\

\rowcolor{baserow}
PDrop
& CVPR'25
& 25.9 & 30.9 & \second{24.2}
& 21.2 & \second{26.7} & \second{19.2}
& 24.1 & 23.7
& \second{29.3\%} \\

\midrule
\rowcolor{routerow}
FastV+Reroute\Route
& Ours
& \second{26.8} & \second{31.1} & 22.9
& \second{21.7} & 26.0 & 18.0
& \second{25.3} & \second{24.1}
& 29.3\% \\

\rowcolor{routerow}
PDrop+Reroute\Route
& Ours
& \best{33.2} & \best{37.6} & \best{31.5}
& \best{27.7} & \best{33.5} & \best{25.1}
& \best{31.0} & \best{29.7}
& \best{37.4\%} \\

\midrule
\multicolumn{11}{c}{\textit{Average Token Reduction} $\downarrow 88.9\%$} \\
\midrule
\rowcolor{baserow}
FastV
& ECCV'24
& 1.6 & 1.6 & 2.2
& 1.7 & 1.7 & 2.6
& 2.0 & 2.3
& 2.4\% \\

\rowcolor{baserow}
PDrop
& CVPR'25
& \second{10.2} & \second{10.9} & \second{9.0}
& \second{7.9} & \second{9.8} & \second{6.7}
& \second{9.9} & \second{9.5}
& \second{11.1\%} \\

\midrule
\rowcolor{routerow}
FastV+Reroute\Route
& Ours
& 6.2 & 5.5 & 5.9
& 4.8 & 4.2 & 4.8
& 6.7 & 6.5
& 6.7\% \\

\rowcolor{routerow}
PDrop+Reroute\Route
& Ours
& \best{16.8} & \best{19.2} & \best{15.2}
& \best{13.9} & \best{16.9} & \best{12.2}
& \best{15.0} & \best{14.9}
& \best{18.6\%} \\

\bottomrule
\end{tabular}%
}
% }

\vspace{0.35em}
\footnotesize{
\colorbox{vanillarow}{Vanilla baseline};
\colorbox{baserow}{Base methods};
\colorbox{routerow}{Reroute variants}. \\
\Route: reroute variant.
Unavailable results are denoted by ``--''.
For RefCOCO and RefCOCO+, A/B denote testA/testB.
Avg. Ratio is the mean score ratio against the vanilla baseline,
computed over subsets where both scores are available.
Schedule details are reported in the appendix.
}
\end{table}

==> tables/qwen35_vg.tex <==
% Required packages:
% \usepackage{booktabs}
% \usepackage[table]{xcolor}
% \usepackage{graphicx}

% ============================================================
% Qwen3.5-9B Hybrid Visual Grounding / RefCOCO Table
% ============================================================

\begin{table}[t]
\centering
\caption{
\textbf{Performance comparison on RefCOCO-series visual grounding benchmarks using
Qwen3.5-9B-Hybrid.} Best and second-best results within each average-token block are
shown in \best{bold} and \second{underlined}, respectively.
}
\label{tab:qwen35_refcoco_main}
\small
% \setlength{\tabcolsep}{3.0pt}
% \renewcommand{\arraystretch}{1.08}
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}llccccccccc@{}}
\toprule
\textbf{Method} & \textbf{Source}
& \multicolumn{3}{c}{\textbf{RefCOCO}}
& \multicolumn{3}{c}{\textbf{RefCOCO+}}
& \multicolumn{2}{c}{\textbf{RefCOCOg}}
& \shortstack[c]{\textbf{Avg.}} \\
\cmidrule(lr){3-5}
\cmidrule(lr){6-8}
\cmidrule(lr){9-10}
& & \textbf{val} & \textbf{A} & \textbf{B}
& \textbf{val} & \textbf{A} & \textbf{B}
& \textbf{val} & \textbf{test}
& \textbf{Ratio}\\
\midrule

\multicolumn{11}{c}{\textit{Average Gated Attention Token (100\%)}} \\
\midrule
\rowcolor{vanillarow}
Vanilla
& Qwen'25
& \best{90.4} & \best{90.7} & \best{85.5}
& \best{80.0} & \best{84.3} & \best{75.7}
& \best{87.3} & \best{86.8}
& \best{100.0\%} \\

\midrule
\multicolumn{11}{c}{\textit{Average Gated Attention Token Reduction} $\downarrow 66.7\%$} \\
\midrule
\rowcolor{baserow}
FastV
& ECCV'24
& 28.7 & 32.5 & 25.6
& 25.2 & 28.3 & 20.3
& 26.3 & 25.6
& 31.1\% \\

\rowcolor{baserow}
PDrop(L8)
& CVPR'25
& 24.9 & 29.0 & 20.3
& 20.3 & 25.3 & 16.1
& 21.2 & 20.7
& 26.0\% \\

\rowcolor{baserow}
PDrop(L2)
& CVPR'25
& 36.4 & 40.4 & 32.4
& 32.7 & 36.1 & 27.4
& 33.7 & 33.4
& 40.0\% \\

\midrule
\rowcolor{routerow}
FastV+Reroute\Route
& Ours
& \best{70.8} & \second{75.1} & \best{64.8}
& \second{60.7} & \second{67.0} & \second{53.9}
& \second{68.5} & \second{68.0}
& \second{77.5\%} \\

\rowcolor{routerow}
PDrop+Reroute\Route
& Ours
& \second{70.0} & \best{76.1} & \second{62.4}
& \best{61.1} & \best{68.6} & \best{54.2}
& \best{69.2} & \best{68.3}
& \best{77.7\%} \\

\midrule
\multicolumn{11}{c}{\textit{Average Gated Attention Token Reduction} $\downarrow 77.8\%$} \\
\midrule
\rowcolor{baserow}
FastV
& ECCV'24
& 18.0 & 22.2 & 15.9
& 14.5 & 18.3 & 12.3
& 16.6 & 15.9
& 19.5\% \\

\rowcolor{baserow}
PDrop
& CVPR'25
& 23.9 & 28.6 & 20.4
& 20.4 & 25.0 & 16.7
& 20.8 & 20.4
& 25.8\% \\

\midrule
\rowcolor{routerow}
FastV+Reroute\Route
& Ours
& \second{51.7} & \second{58.4} & \second{44.6}
& \second{42.3} & \second{49.7} & \second{35.7}
& \second{50.2} & \second{49.6}
& \second{55.9\%} \\

\rowcolor{routerow}
PDrop+Reroute\Route
& Ours
& \best{54.9} & \best{62.7} & \best{47.0}
& \best{46.4} & \best{53.5} & \best{38.0}
& \best{52.9} & \best{52.2}
& \best{59.7\%} \\

\midrule
\multicolumn{11}{c}{\textit{Average Gated Attention Token Reduction} $\downarrow 88.9\%$} \\
\midrule
\rowcolor{baserow}
FastV
& ECCV'24
& 12.4 & 14.7 & 12.3
& 6.8 & 6.8 & 5.8
& 8.3 & 8.1
& 10.9\% \\

\rowcolor{baserow}
PDrop
& CVPR'25
& \second{19.5} & \second{23.8} & \second{15.7}
& \second{14.2} & \second{17.8} & \second{10.0}
& \second{15.8} & \second{15.5}
& \second{19.3\%} \\

\midrule
\rowcolor{routerow}
FastV+Reroute\Route
& Ours
& 14.2 & 15.0 & 13.2
& 8.8 & 9.4 & 7.6
& 11.9 & 11.6
& 13.4\% \\

\rowcolor{routerow}
PDrop+Reroute\Route
& Ours
& \best{35.0} & \best{41.1} & \best{27.8}
& \best{27.8} & \best{34.8} & \best{22.2}
& \best{33.7} & \best{33.8}
& \best{37.4\%} \\

\bottomrule
\end{tabular}%
% }

\vspace{0.35em}
\footnotesize{
\colorbox{vanillarow}{Vanilla baseline};
\colorbox{baserow}{Base methods};
\colorbox{routerow}{Reroute variants}. \\
\Route: reroute variant.
Unavailable results are denoted by ``--''.
For RefCOCO and RefCOCO+, A/B denote testA/testB.
Avg. Ratio is the mean score ratio against the vanilla baseline,
computed over subsets where both scores are available.
Schedule details are reported in the appendix.
}
\end{table}
